Standing Firm in 5G: A Single-Round, Dropout-Resilient Secure Aggregation for Federated Learning

Federated learning (FL) is well-suited to 5G networks, where many mobile devices generate sensitive edge data. Secure aggregation protocols enhance privacy in FL by ensuring that individual user updates reveal no information about the underlying client data. However, the dynamic and large-scale nature of 5G-marked by high mobility and frequent dropouts-poses significant challenges to the effective adoption of these protocols. Existing protocols often require multi-round communication or rely on fixed infrastructure, limiting their practicality. We propose a lightweight, single-round secure aggregation protocol designed for 5G environments. By leveraging base stations for assisted computation and incorporating precomputation, key-homomorphic pseudorandom functions, and t-out-of-k secret sharing, our protocol ensures efficiency, robustness, and privacy. Experiments show strong security guarantees and significant gains in communication and computation efficiency, making the approach well-suited for real-world 5G FL deployments.

==> algo/algos.tex <==

\begin{algorithm*}[t]\caption{Setup}\label{alg:sysSetup}
\small
\raggedright{\textbf{Input:} All parties are provided with the security parameter $\kappa $, the number of assisting nodes $k$, a key encapsulation protocol $\kem=\{\sgnkeygen, \kemenc, \kemdec\}$,
 a digital signature scheme with precomputation $\Pi$: $(\sgnkeygen,\precomputesgn,\presgnsign,\sgnverify)$,  
 a secret sharing scheme $\sss = \{ \sssplit, \ssrecover\}$,
 instantiated using the security parameter $\kappa$, and {\color{red} a key-homomorphic pseudorandom function $\khprf$}. 

\textbf{Output:} All the entities generate their key exchange, signature  key pairs, as well as precomputed signing parameter list $\mathcal{LS}$.

All the users receive the public keys of all the  assisting nodes $\langle(\pk^{\node_1}_\Pi, \dots, \pk^{\node_k}_\Pi),(\pk^{\node_1}_\kem, \dots, \pk^{\node_k}_\kem)\rangle$, and shared secret seed $\x^{\user_i}_{\node_j}$ for each assisting node $\node_j$.
% 
All the assisting nodes receive the public keys of all the  participating users $(\pk^{\user_1}_\Pi, \dots, \pk^{\user_n}_\Pi)$, and a shared secret seed $\x^{\node_j}_{\user_i}$ with each user $\user_i$.  
The aggregation server  \agg~receives the public keys of all the users and  assisting nodes $\langle(\pk^{\user_1}_\Pi, \dots, \pk^{\user_k}_\Pi),(\pk^{\node_1}_\Pi, \dots, \pk^{\node_k}_\Pi)\rangle$.} 
Lastly, all the users and assisting nodes generate the precomputed mask lists $\mathcal{MS}$. \\





\hrulefill \vspace{-1mm}


 
\textbf{Phase} 1 \textbf{(KeyGen and Advertise)}
\vspace{-2mm}

\hrulefill


All the communications below are conducted via an authenticated channel (similar to xxx)
\begin{algorithmic}[1] 


\item Each assisting node $\node_j$ generates its key pair(s) $(\sk^{\node_j}_\Pi,\pk^{\node_j}_\Pi)\gets\Pi.\sgnkeygen(\kappa)$ and$(\sk^{\node_j}_\kem,\pk^{\node_j}_\kem)\gets\kem.\kagen(\kappa)$  and sends $(\pk^{\node_j}_\Pi, \pk^{\node_j}_\kem)$  to the $n$ users and sends $\pk^{\node_j}_\Pi$ the aggregation server.  

\item Upon receiving $\pk^{\node_j}_\kem$ from $\node_j$,  each user $\user_i$ computes and encapsulate a shared secret by $(\x_{\node_j}^{\user_i}, c_{\node_j}^{\user_i})\gets\kem.\kemenc(\pk_\kem^{\node_j})$. It then generates its key pair(s) $(\sk^{\user_i}_\Pi,\pk^{\user_i}_\Pi)\gets\Pi.\sgnkeygen(\kappa)$  and sends  $\pk^{\user_i}_\Pi$ and   $c_{\node_j}^{\user_i}$ to $\node_j$ to the $k$ assisting nodes and $\pk^{\user_i}_\Pi$ to the aggregation server.  


% Each user $\user_i$ generates its key pair(s) \mal{\uline{$(\sk^{\user_i}_\Pi,\pk^{\user_i}_\Pi)\gets\Pi.\sgnkeygen(\kappa)$ }}  \mal{\uline{and sends  $\mal{\pk^{\user_i}_\Pi}$ to the $k$ assisting nodes and $\pk^{\user_i}_\Pi$ to the aggregation server}}. 
 






% \item Upon receiving $\pk^{\user_i}_\kem$ from $\user_i$,  each assisting node $\node_j$ computes and sends a shared secret seed $\x^{\node_j}_{\user_i}$ and encapsulate it by $c^{\node_j}_{\user_i}\gets\kemenc(\x^{\node_j}_{\user_i},\pk_\kem^{\node_j})$ and sends  $c^{\node_j}_{\user_i}$ to $\user_i$.

% \yiwei{}


 
% \item Upon receiving $c^{\node_j}_{\user_i}$  from the assisting node $\node_j$, the user $\user_i$ computes retrieves the shared secret  
% $ \x^{\node_j}_{\user_i} \gets \kemdec(c^{\node_j}_{\user_i}, \sk_\kem^{\node_j})$. 

% \yiwei{
\item 
% Upon receiving $c_{\node_j}^{\user_i}$  from the assisting node $\node_j$, the user $\user_i$ 
Upon receiving $c_{\node_j}^{\user_i}$ from the the user $\user_i$, the assisting node $\node_j$
computes and retrieves the shared secret  
$\x_{\node_j}^{\user_i} \gets \kem.\kemdec(c_{\node_j}^{\user_i}, \sk_\kem^{\node_j})$
 

\item The aggregation server \agg~generates a key pair $(\sk^\mathtt{S}_\Pi,\pk^\mathtt{S}_\Pi)\gets\Pi.\sgnkeygen(1^\kappa)$ and sends $\pk^\mathtt{S}_\Pi$ to the users.


\item All the entities perform the precomputation to get a list $\mathcal{LS}$ with $N$ groups of pre-computated parameters for optimizing further signing operations: $\mathcal{LS}_{\node_j} \gets \precomputesgn(\sk_{\node_j}, N)$, $\mathcal{LS}_{\user_i} \gets \precomputesgn(\sk_{\user_i}, N)$, $\mathcal{LS}_{\agg} \gets \precomputesgn(\sk_\agg, N)$.


\item Each user $\user_i$ computes a list $\mathcal{MS}_{\user_i}^{\node_j}$ for each assisting node $\node_j$, with $T$ groups of masks: $\mathcal{MS}_{\user_i}^{\node_j}$[$t$] = $\prf(\x_{\user_i}^{\node_j},t)$ for $t\in[1,\dots,T]$. Similarly, each assisting node $\node_j$ computes a list $\mathcal{MS}_{\node_j}^{\user_i}$: $\mathcal{MS}_{\node_j}^{\user_i}$[$t$] = $\khprf(\x_{\node_j}^{\user_i},t)$ for $t\in[1,\dots,T]$.

\item {\color{red} Each assisting node $\node_j$ generates $t_{ss}$-out-of-(k-1) secret shares: $x_{\node_j}^{\user_i}.ss_1, ..., x_{\node_j}^{\user_i}.ss_{k-1} \gets \sss.\sssplit(x_{\node_j}^{\user_i}, t_{ss}, k)$, and sends one share to each other assisting node with signatures.}

% \item \mal{The aggregation server \agg~generates a key pair $(\sk^\mathtt{S}_\Pi,\pk^\mathtt{S}_\Pi)\gets\Pi.\sgnkeygen(\kappa)$ and sends $\pk^\mathtt{S}_\Pi$ to the $k$ assisting nodes.} 
\end{algorithmic}

\end{algorithm*}


\begin{algorithm*}[!t]\caption{Aggregation}\label{alg:sysAgg}
\small
\raggedright{\textbf{Input:} The iteration $t$, a user calculated model update $\vec{w}^{\user_i}_t$, a keyed pseudorandom function $\prf $, {\color{red} a key-homomorphic pseudorandom function $\khprf$}, a digital signature scheme $\Pi$,   the secret seeds $\x$ (shared between the users and the nodes), the signature key pair of the users and the assisting nodes, as well as the precomputed signing parameter list $\mathcal{LS}$ of all entities and the precomputed mask list $\mathcal{MS}$ of the users and the assisting nodes. 
 

\textbf{Output:} The final model update $\vec{w}_t \in \mathcal{M}^d$. \\


 
\hrulefill \vspace{-1mm}

\textbf{Phase} 1 \textbf{(Masking Updates)}}

\vspace{-2mm}


\hrulefill 


\begin{algorithmic}[1]


\State The user compute the local  update $\Vec{w}^{\user_i}_{t}$ for iteration $t$

\State The user $\user_i$ first gets the mask $\mathcal{MS}_{\user_i}^{\node_j}$[$t$] for iteration $t$, and then computes $\Vec{a}^{\user_i}_{t}=\sum_{j=1}^k$$\mathcal{MS}_{\user_i}^{\node_j}$[$t$] 
and the masked update $\vec{y}^{\user_i}_{t}=\vec{w}^{\user_i}_{t}+\Vec{a}^{\user_i}_{t}$. 


\State The user sets $m=(t,\vec{y}^{\user_i}_{t})$ and $m'=(t)$, computes signatures $\sigma^{\user_i}_{\agg} \gets \Pi.\presgnsign(\sk^{\user_i}_\Pi,m, \mathcal{LS}_{\user_i})$ and $\sigma^{\user_i}_{\node_j} \gets \Pi.\presgnsign(\sk^{\user_i}_\Pi,m', \mathcal{LS}_{\user_i})$ and sends $(m,\sigma^{\user_i}_{\agg})$ and $(m',\sigma^{\user_i}_{\node_j})$ to the aggregation server and the assisting node $\node_j $ (for $j\in[1,\dots,k]$), respectively. 

% \yiwei{Don't have to send $m'$ to the assisting nodes.}

% \State {\color{red} Each node $\node_j$ sets $m_j=(t, \mathcal{MS}_{\node_j}^{\user_1}[t]_{j'}, ..., \mathcal{MS}_{\node_j}^{\user_n}[t]_{j'})$  and sends $m_j$ to the assisting nodes $\node_{j'}$ for $j'\in[1,\dots,k]$ and $j \neq j'$.}

\end{algorithmic}

 
 \hrulefill \vspace{-1mm}

 
\textbf{Phase} 2 \textbf{(Aggregate Updates)}
\vspace{-2mm}

\hrulefill 

 
\begin{algorithmic}[1]
\State Upon receiving $(m',\sigma^{\user_i}_{\node_j})$
% , $\node_j$  receives $(m'\mal{,\sigma^{\user_i}_{\node_j}})$ 
from all the  users in the system, $\node_j$ checks if  $ \Pi.\sgnverify(\pk_\Pi^{\user_i},m',\sigma^{\user_i}_{\node_j} ) \stackrel{?}{=} 1$ holds, it adds the user to its user list $\mathcal{L}_{j,t}$. 

\State Each assisting node checks if  {$|\mathcal{L}_{j,t}|\geq \alpha\ppp_H$}, 
% it computes  $\Vec{a}^{\node_j}_{t}=\sum_{i=1}^{|\mathcal{L}_{j,t}|}\prf(\x^{\node_j}_{\user_i},t)$, 
it gets $\mathcal{MS}_{\node_j}^{\user_i}$[$t$], computes $\Vec{a}^{\node_j}_{t}=\sum_{i=1}^{|\mathcal{L}_{j,t}|}$$\mathcal{MS}_{\node_j}^{\user_i}$[$t$],
sets $m^{\prime\prime}=(t,|\mathcal{L}_{j,t}|,\Vec{a}^{\node_j}_t)$ and $\sigma^{\node_i}_{\agg} \gets \Pi.\presgnsign(\sk^{\node_j}_\Pi,m'', \mathcal{LS}_{\node_j})$  and sends $(m'',\sigma^{\node_j}_{\agg})$ to the aggregation server \agg. 


\State Upon receiving $(m,\sigma^{\user_i}_{\agg})$, \agg~first checks if 
$ \Pi.\sgnverify(\pk_\Pi^{\user_i},m,\sigma^{\user_i}_{\agg} )\stackrel{?}{=}  1$ holds, it adds $\user_i$ to its user list $\mathcal{L}_{\agg,\user,t}$. 




% \State The aggregation server verifies the message-signature pairs $(m,\sigma^{\user_i}_{\agg})$ from the users, for all the valid pairs,  it  adds the user to its user list $\mathcal{L}_{\agg,t}$. 
\State Next, \agg~checks if   $  \Pi.\sgnverify(\pk_\Pi^{\node_j},m'',\sigma^{\node_j}_{\agg} )\stackrel{?}{=}  1$ holds   for $j\in[1,\dots,k]$. It then checks if  $|\mathcal{L}_{\agg,\user,t}|= |\mathcal{L}_{1,t}| =\dots = |\mathcal{L}_{k,t}|$. {\color{red} If both conditions hold, it adds $\node_j$ to its node list $\mathcal{L}_{\agg,\node,t}$.}

\State {\color{red} \agg~gets the list $\mathcal{L}_{\agg,\node_{off},t}$ including offline assisting nodes, i.e., $\node_j \notin \mathcal{L}_{\agg,\node,t}$ for each $\node_j  \in \mathcal{L}_{\agg,\node_{off},t}$.}

\State {\color{red} \agg~sets $m = (t,  \mathcal{L}_{\agg,\node_{off},t}, \mathcal{L}_{\agg,\user,t})$ and sends $m$ to each online assisting node $\node_j \in \mathcal{L}_{\agg,\node,t}$.}

{\color{red} \textbf{Method 1}}

\State {\color{red} Each online assisting node $\node_j \in \mathcal{L}_{\agg,\node,t}$ calculates the mask of secret share of offline nodes $\khprf(x_{\node_{j'}}^{\user_i}.ss_{j})$ for each offline node $\node_{j'}$, and send it to each other assisting node. Then the online assisting nodes can recover the mask of offline nodes: $\khprf(x_{\node_{j'}}^{\user_i}) = \sss.\ssrecover(\khprf(x_{\node_{j'}}^{\user_i}.ss_j)$ for $j \in \mathcal{L}_{\agg,\node,t}$, $j'\in \mathcal{L}_{\agg,\node_{off},t})$}.

\State {\color{red} Online assisting nodes then calculate the sum of masks of offline nodes: $\sum(\khprf(x_{\node_{j'}}^{\user_i}))$, and then send it to the \agg.}

\State {\color{red} \agg receives the sum of masks of offline nodes: $\sum_{j' \in \mathcal{L}_{\agg,\node_{off},t}} \Vec{a}^{\node_{j'}}_t = \sum(\khprf(x_{\node_{j'}}^{\user_i}))$ }

% \State {\color{red} Each online assisting node $\node_j \in \mathcal{L}_{\agg,\node,t}$ calculates the sum of secret share of offline nodes: $\mathcal{MM}_j = \sum_{i=1}^{|\mathcal{L}_{\agg,\user,t}|} \sum_{j' \in \mathcal{L}_{\agg,\node_{off},t}} \mathcal{MS}_{\node_{j'}}^{\user_i}[t]_{j}$
% sets $m = (t, \mathcal{MM}_j$), and sends $m$ to \agg.}

{\color{blue} \textbf{Method 2}}
\State {\color{blue} Each online assisting node $\node_j \in \mathcal{L}_{\agg,\node,t}$ calculates the mask of secret share of offline nodes $\khprf(x_{\node_{j'}}^{\user_i}.ss_{j})$ for each offline node $\node_{j'}$, and send it to \agg}.

\State {\color{blue} \agg~recovers the sum of masks of offline assisting nodes: $\sum_{j' \in \mathcal{L}_{\agg,\node_{off},t}} \Vec{a}^{\node_{j'}}_t = \sss.\ssrecover(\khprf(x_{\node_{j'}}^{\user_i}.ss_{j})$ for $j \in \mathcal{L}_{\agg,\node,t}$, $j'\in \mathcal{L}_{\agg,\node_{off},t})$)}
% \sum_{j \in \mathcal{L}_{\agg,\node,t}} \mathcal{MM}_j$.}

\State {\color{red} \agg~computes and broadcasts the final update as $\vec{w}_t=\sum_{i=1}^{|\mathcal{L}_{\agg,\user,t}|}\vec{y}^{\user_i}_{t} - \sum_{j \in \mathcal{L}_{\agg,\node,t}}\Vec{a}^{\node_j}_t - \sum_{j' \in \mathcal{L}_{\agg,\node_{off},t}} \Vec{a}^{\node_{j'}}_t$.} 

% \State \agg~computes and broadcasts the final update as $\vec{w}_t=\sum_{i=1}^{|\mathcal{L}_{\agg,t}|}\vec{y}^{\user_i}_{t}-\sum_{j=1}^k\Vec{a}^{\node_j}_t$. 

 

 
 \end{algorithmic}
\end{algorithm*}




\setlength{\floatsep}{0.1cm}


The following describes KHPRF:

\begin{algorithm}
\caption{Key Homomorphic Pseudorandom Function (KH-PRF)}
\label{alg:khprf}
\begin{algorithmic}[1]
% \Require Secret key $k$, input $x$, hash function $h(x)$
% \Ensure Pseudorandom output $y$
\State Require Secret key $k$, input $x$, hash function $h(x)$
\State Ensure Pseudorandom output $y$

\State \textbf{Compute} the hash of the input:
\State \hspace{1cm} $v \gets h(x)$
\State \textbf{Multiply} by the secret key:
\State \hspace{1cm} $y \gets k \cdot v$
\State Return $y$
\end{algorithmic}

\end{algorithm}


==> discussion.tex <==
\section{Discussion}
\imtiaz{I think too much future work, see Slack note}
Our protocol uses $t$-out-of-$k$ secret sharing and key-homomorphic PRFs to protect local user updates in 5G-based FL, addressing moderate failures arising from high user mobility and frequent handovers. However, three key challenges and future directions merit further investigation:

\noindent
\textbf{Adaptive Base Station Selection.} Selecting BSs within a UE’s coverage to collectively recover the global update is complicated by user mobility. An ML-based method that adaptively identifies the most suitable BSs could balance communication overhead and security as UEs move.

\noindent
\textbf{Share Reassignment and Revocation.} When a BS becomes unreachable or proves malicious, secret splits must be quickly reassigned to a newly added BS, and the compromised BS must be revoked. Such a mechanism protects against incorrect mask shares that would otherwise disrupt global model aggregation.

\noindent
\textbf{$t$-out-of-$k$ Secret Sharing for BS Collusion Resistance.} The threshold approach inherently prevents collusion by requiring multiple honest BSs to reconstruct the masks. Future work may explore more adaptive or robust threshold schemes—potentially coupled with zero-knowledge proofs—to handle extreme churn or highly adversarial environments.

% \paragraph{Adaptive Base Station Selection.} In the current design, a chosen subset of BSs within a certain region collectively “remove the mask” to recover the aggregated results. Yet, selecting which BSs should participate is non-trivial, especially given the dynamic mobility of UEs: the set of BSs within a UE’s range may shift frequently. As a result, an intriguing research direction is to develop a data-driven or ML-based framework for BS selection that adaptively responds to real-time mobility and network conditions. Such an approach would help balance communication overheads and maintain secure, efficient aggregation.

% \paragraph{Share Reassignment and Revocation.} Because UEs can migrate to new BSs at any time, a critical challenge lies in securely redistributing the secret splits among newly added BSs and revoking them from the original BSs. This mechanism would not only ensure continuity when a BS goes offline or becomes unreachable but also offer a strategy to mitigate malicious or compromised BSs. If a BS submits an incorrect or inconsistent mask share, the core network aggregator can pinpoint the source of failure and immediately launch a revocation procedure. Reassigning the compromised BS’s secret splits to a trusted replacement would maintain the integrity of future aggregations.

% \paragraph{$t$-out-of-$k$ Secret Sharing for BS Collusion Resistance.} Finally, our use of $t$-out-of-$k$ secret sharing inherently safeguards against collusion attacks by requiring cooperation among at least $t$ honest BSs to reconstruct the global mask. This threshold-based strategy remains robust under moderate adversarial settings. In more extreme threat models with highly collusive or rapidly changing sets of BSs, extending the secret sharing scheme (e.g., by dynamically adjusting the threshold or integrating zero-knowledge proofs) would further enhance security while balancing the added computation and communication overhead.


==> related.tex <==
\section{Related Works}

\subsection{Integrating FL into 5G}


\subsection{Protections}

there are some protections in FL such as secure aggregation

there are also some works to protect FL-5G applications.


But they don't/can't solve node dropout problems



==> tables/efficiency.tex <==
\begin{table}[t]
\centering
\caption{Performance Comparison.}
\label{tab:efficiency}
\begin{tabular}{|C{1cm}|C{1cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|}
% \toprule
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{Device Type}}} & \multicolumn{3}{c|}{\textbf{Computation Cost (ms)}} \\ \cline{3-5} 
\multicolumn{2}{|c|}{} & \textbf{Ours} & \textbf{\eseafl} & \textbf{\flamingo} \\ \hline 
\multirow{2}{*}{\textbf{$CNAF_{FL}$}} & Setup & - & - & 1.37  \\ \cline{2-5}
& Agg. & 0.11 & 1.08 & 7.56 \\ \hline
\multirow{2}{*}{\textbf{$BS$}} & Setup & - & 0.81 & 5.21 \\ \cline{2-5}
& Agg. & 0.25 & 1.57 & 1.28  \\ \hline
\multirow{2}{*}{\textbf{$UE$}} & Setup & 0.39 & 0.26 & 0.07 \\ \cline{2-5}
& Agg. & 0.13 & 0.87 & 26.44 \\ \hline
\multicolumn{2}{|c|}{\textbf{Total Agg.}} & 0.49 & 3.52 & 35.28 \\ \hline

\end{tabular}

\vspace{5pt}

\begin{tabular}{|C{1cm}|C{1cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|}
% \toprule
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{Device Type}}} & \multicolumn{3}{c|}{\textbf{Communication Cost (KB)}} \\ \cline{3-5} 
\multicolumn{2}{|c|}{} & \textbf{Ours} & \textbf{\eseafl} & \textbf{\flamingo} \\ \hline 
\multirow{2}{*}{\textbf{$CNAF_{FL}$}} & Setup & - & - & 2.72 \\ \cline{2-5}
& Agg. & 2502.17 & 2501.00 & 2540.37 \\ \hline
\multirow{2}{*}{\textbf{$BS$}} & Setup & - & 0.57 & -  \\ \cline{2-5}
& Agg. & 0.06 & 312.70 & 2.11 \\ \hline
\multirow{2}{*}{\textbf{$UE$}} & Setup & 0.35 & 0.21 & -\\ \cline{2-5}
& Agg. & 312.63 & 312.75 & 319.66  \\ \hline
\multicolumn{2}{|c|}{\textbf{Total Agg.}} & 2814.86 & 3126.45 & 2861.77  \\ \hline

\end{tabular}
% \begin{tablenotes}
% \item The best efficiency is marked as {\textcolor{red}{red color}}.
% % \flamingo without encryption and signuares.
% \end{tablenotes}
\end{table}

